A scalable multi-step least squares method for network identification with unknown disturbance topology

Identification methods for dynamic networks typically require prior knowledge of the network and disturbance topology, and often rely on solving poorly scalable non-convex optimization problems. While methods for estimating network topology are available in the literature, less attention has been paid to estimating the disturbance topology, i.e., the (spatial) noise correlation structure and the noise rank in a filtered white noise representation of the disturbance signal. In this work we present an identification method for dynamic networks, in which an estimation of the disturbance topology precedes the identification of the full dynamic network with known network topology. To this end we extend the multi-step Sequential Linear Regression and Weighted Null Space Fitting methods to deal with reduced rank noise, and use these methods to estimate the disturbance topology and the network dynamics in the full measurement situation. As a result, we provide a multi-step least squares algorithm with parallel computation capabilities and that rely only on explicit analytical solutions, thereby avoiding the usual non-convex optimizations involved. Consequently we consistently estimate dynamic networks of Box Jenkins model structure, while keeping the computational burden low. We provide a consistency proof that includes path-based data informativity conditions for allocation of excitation signals in the experimental design. Numerical simulations performed on a dynamic network with reduced rank noise clearly illustrate the potential of this method.

==> main.tex <==
\begin{thebibliography}{10}

\bibitem{Araki}
M.~{Araki} and M.~{Saeki}.
\newblock A quantitative condition for the well-posedness of interconnected
  dynamical systems.
\newblock {\em IEEE Transactions on Automatic Control}, 28(5):569--577, 1983.

\bibitem{bach2011convex}
F.~Bach, R.~Jenatton, J.~Mairal, G.~Obozinski, et~al.
\newblock Convex optimization with sparsity-inducing norms.
\newblock {\em Optimization for Machine Learning}, 5:19--53, 2011.

\bibitem{bolstad2011causal}
A.~Bolstad, B.D. Van~Veen, and R.~Nowak.
\newblock Causal network inference via group sparse regularization.
\newblock {\em IEEE Transactions on Signal Processing}, 59(6):2628--2641, 2011.

\bibitem{BOMBOIS_hal_2021}
X.~Bombois and H.~Hjalmarsson.
\newblock Network topology detection via uncertainty analysis of an identified
  static model.
\newblock {\em IFAC-PapersOnLine}, 54(7):595--600, 2021.
\newblock 19th IFAC Symposium on System Identification SYSID 2021.

\bibitem{boyd2011Glasso}
S.~Boyd, N.~Parikh, and E.~Chu.
\newblock {\em Distributed optimization and statistical learning via the
  alternating direction method of multipliers}.
\newblock Now Publishers Inc, 2011.

\bibitem{CambaMendez&Kapetanios:09}
G.~Camba-M\'{e}ndez and G.~Kapetanios.
\newblock Statistical tests and estimators of the rank of a matrix and their
  applications in econometric modelling.
\newblock {\em Econometrics Reviews}, 28(6):581--611, 2009.

\bibitem{Cao&Picci&Lindquist_id:21}
W.~Cao, G.~Picci, and A.~Lindquist.
\newblock Identification of low rank vector processes, 2021.
\newblock ArXiv: 2111.10899, Submitted for publication.

\bibitem{chiuso2012bayesian}
A.~Chiuso and G.~Pillonetto.
\newblock A bayesian approach to sparse dynamic network identification.
\newblock {\em Automatica}, 48(8):1553--1565, 2012.

\bibitem{Dankers_SLR}
A.G. Dankers.
\newblock Optimization method for obtaining estimates in a dynamic network.
\newblock Technical note, 2019.

\bibitem{Dankers:15EIV}
A.G. {Dankers}, P.M.J. {Van den Hof}, X.~Bombois, and P.S.C. Heuberger.
\newblock Errors-in-variables identification in dynamic networks —
  consistency results for an instrumental variable approach.
\newblock {\em Automatica}, 62:39 -- 50, 2015.

\bibitem{DANKERS2012structure}
A.G. Dankers, P.M.J. {Van den Hof}, P.S.C. Heuberger, and X.~Bombois.
\newblock Dynamic network structure identification with prediction error
  methods - basic examples.
\newblock {\em IFAC Proceedings Volumes}, 45(16):876 -- 881, 2012.
\newblock 16th IFAC Symposium on System Identification.

\bibitem{Dankers&etal_TAC:16}
A.G. Dankers, P.M.J. Van~den Hof, P.S.C. Heuberger, and X.~Bombois.
\newblock Identification of dynamic models in complex networks with prediction
  error methods: Predictor input selection.
\newblock {\em IEEE Transactions on Automatic Control}, 61(4):937--952, 2016.

\bibitem{Deistler2010}
M.~Deistler, B.D.O. Anderson, A.~Filler, C.~Zinner, and W.~Chen.
\newblock Generalized linear dynamic factor models: An approach via singular
  autoregressions.
\newblock {\em European Journal of Control}, 16(3):211--224, 2010.

\bibitem{Deistler2015}
M.~Deistler, W.~Scherrer, and B.D.O. Anderson.
\newblock The structure of generalized linear dynamic factor models.
\newblock In J.~Beran, Y.~Feng, and H.~Hebbel, editors, {\em Empirical Economic
  and Financial Research: Theory, Methods and Practice}, pages 379--400.
  Springer International Publishing, Cham, 2015.

\bibitem{Dimovska2017}
M.~Dimovska and D.~Materassi.
\newblock Granger-causality meets causal inference in graphical models:
  Learning networks via non-invasive observations.
\newblock In {\em 2017 IEEE 56th Annual Conference on Decision and Control
  (CDC)}, pages 5268--5273, 2017.

\bibitem{morsm2016}
N.~Everitt, M.~Galrinho, and H.~Hjalmarsson.
\newblock Open-loop asymptotically efficient model reduction with the
  {S}teiglitz–{M}cbride method.
\newblock {\em Automatica}, 89:221 -- 234, 2018.

\bibitem{WNSF_stef}
S.J.M. Fonken, M.~Ferizbegovic, and H.~Hjalmarsson.
\newblock Consistent identification of dynamic networks subject to white noise
  using weighted null-space fitting.
\newblock {\em IFAC-PapersOnLine}, 53-2:46--51, 2020.
\newblock Proc. 21st IFAC World Congress, Berlin, Germany.

\bibitem{Galrinho_Para_WNSF_2019}
M.~{Galrinho}, C.~Rojas, and H.~Hjalmarsson.
\newblock Parametric identification using {W}eighted {N}ull-{S}pace {F}itting.
\newblock {\em IEEE Transactions on Automatic Control}, 64(7):2798--2813, 2019.

\bibitem{Gevers&etal_sysid:18}
M.~Gevers, A.S. Bazanella, and G.~Vian~da Silva.
\newblock A practical method for the consistent identification of a module in a
  dynamical network.
\newblock {\em IFAC-PapersOnLine}, 51-15:862--867, 2018.
\newblock Proc. 18th IFAC Symp. System Identification (SYSID2018).

\bibitem{brain_netw}
P.~Hagmann, L.~Cammoun, X.~Gigandet, R.~Meuli, C.~J Honey, Van~J. Wedeen, and
  O.~Sporns.
\newblock Mapping the structural core of human cerebral cortex.
\newblock {\em PLOS Biology}, 6(7):1--15, 07 2008.

\bibitem{hajian2013ROC}
K.~Hajian-Tilaki.
\newblock Receiver operating characteristic (roc) curve analysis for medical
  diagnostic test evaluation.
\newblock {\em Caspian Journal of Internal Medicine}, 4(2):627, 2013.

\bibitem{Bio_net}
R.~Hickman, M.C. Van~Verk, A.J.H. Van~Dijken, M.P. Mendes, I.A. Vroegop-Vos,
  L.~Caarls, M.~Steenbergen, I.~Van~der Nagel, G.J. Wesselink, A.~Jironkin,
  A.~Talbot, J.~Rhodes, M.~De~Vries, R.C. Schuurink, K.~Denby, C.M.J. Pieterse,
  and S.C.M. Van~Wees.
\newblock Architecture and dynamics of the jasmonic acid gene regulatory
  network.
\newblock {\em The Plant Cell}, 29(9):2086--2105, 2017.

\bibitem{Bayes_factors}
R.E. Kass and A.E. Raftery.
\newblock Bayes factors.
\newblock {\em Journal of the American Statistical Association},
  90(430):773--795, 1995.

\bibitem{ljung99}
L.~Ljung.
\newblock {\em {System Identification. Theory for the User, 2nd ed.}}
\newblock Prentice-Hall, 1999.

\bibitem{Wahlberg_Ljung_As_Prop}
L.~{Ljung} and B.~Wahlberg.
\newblock Asymptotic properties of the least-squares method for estimating
  transfer functions and disturbance spectra.
\newblock {\em Advances in Applied Probability}, 24(2):412--440, 1992.

\bibitem{materassi2010topological}
D.~Materassi and G.~Innocenti.
\newblock Topological identification in networks of dynamical systems.
\newblock {\em IEEE Transactions on Automatic Control}, 55(8):1860--1871, 2010.

\bibitem{materassi2012problem}
D.~Materassi and M.V. Salapaka.
\newblock On the problem of reconstructing an unknown topology via locality
  properties of the wiener filter.
\newblock {\em IEEE Transactions on Automatic Control}, 57(7):1765--1777, 2012.

\bibitem{Materassi&Salapaka:20}
D.~Materassi and M.V. Salapaka.
\newblock Signal selection for estimation and identification in networks of
  dynamic systems: a graphical model approach.
\newblock {\em IEEE Transactions on Automatic Control}, 65(10):4138--4153,
  october 2020.

\bibitem{Materassi_Relations}
D.~{Materassi}, M.V. {Salapaka}, and L.~{Giarrè}.
\newblock Relations between structure and estimators in networks of dynamical
  systems.
\newblock {\em Proceedings of the IEEE Conference on Decision and Control
  (CDC)}, pages 162--167, 12 2011.

\bibitem{pagani_powergrid}
G.A. Pagani and M.~Aiello.
\newblock The power grid as a complex network: A survey.
\newblock {\em Physica A: Statistical Mechanics and its Applications},
  392(11):2688--2700, 2013.

\bibitem{Ramaswamy&etal_Autom:21}
K.R. Ramaswamy, G.~Bottegal, and P.M.J. Van~den Hof.
\newblock Learning linear models in a dynamic network using regularized
  kernel-based methods.
\newblock {\em Automatica}, 129(109591), July 2021.

\bibitem{Ramaswamy&etal_TAC:21}
K.R. Ramaswamy and P.M.J. Van~den Hof.
\newblock A local direct method for module identification in dynamic networks
  with correlated noise.
\newblock {\em IEEE Transactions on Automatic Control}, 66(11):3237--3252,
  November 2021.

\bibitem{schwarz1978estimating}
G.~Schwarz.
\newblock Estimating the dimension of a model.
\newblock {\em The annals of statistics}, pages 461--464, 1978.

\bibitem{shi2019bayesian}
S.~Shi, G.~Bottegal, and P.M.J. {Van den Hof}.
\newblock Bayesian topology identification of linear dynamic networks.
\newblock In {\em 2019 18th European Control Conference (ECC)}, pages
  2814--2819, 2019.

\bibitem{VandenHof2013}
P.M.J. Van~den Hof, A.G. Dankers, P.S.C. Heuberger, and X.~Bombois.
\newblock Identification of dynamic models in complex networks with prediction
  error methods: basic methods for consistent module estimates.
\newblock {\em Automatica}, 49(10):2994--3006, 2013.

\bibitem{Hof2020path}
P.M.J. Van~den Hof and K.R. Ramaswamy.
\newblock Path-based data-informativity conditions for single module
  identification in dynamic networks.
\newblock In {\em Proc. 59th IEEE Conf. on Decision and Control (CDC)}, pages
  4354--4359, Jeju Island, Republic of Korea, 2020. IEEE.

\bibitem{hof_karthik_sur:21a}
P.M.J. {Van den Hof} and K.R. Ramaswamy.
\newblock Learning local modules in dynamic networks.
\newblock In {\em Proceedings of the 3rd Conference on Learning for Dynamics
  and Control}, volume 144 of {\em Proc. Machine Learning Research}, pages
  176--188, 2021.

\bibitem{Woude1991graph}
J.W. Van~der Woude.
\newblock A graph-theoretic characterization for the rank of the transfer
  matrix of a structured system.
\newblock {\em Mathematics of Control, Signals and Systems}, 4(1):33--40, 1991.

\bibitem{veedu2020topology}
M.S. Veedu and M.V. Salapaka.
\newblock Topology identification under spatially correlated noise, 2020.
\newblock ArXiv:2012.04175.

\bibitem{WASSERMAN200092}
L.~Wasserman.
\newblock Bayesian model selection and model averaging.
\newblock {\em Journal of Mathematical Psychology}, 44(1):92 -- 107, 2000.

\bibitem{Harm_SLS}
H.H.M. {Weerts}, M.~Galrinho, G.~Bottegal, H.~Hjalmarsson, and P.M.J. {Van den
  Hof}.
\newblock A {S}equential {L}east {S}quares algorithm for {ARMAX} dynamic
  network identification.
\newblock {\em IFAC-PapersOnLine}, 51(15):844--849, 2018.

\bibitem{weerts_rank_reduced}
H.H.M. Weerts, P.M.J. {Van den Hof}, and A.G. Dankers.
\newblock Identification of dynamic networks with rank-reduced process noise.
\newblock {\em IFAC-PapersOnLine}, 50(1):10562--10567, 2017.

\bibitem{WEERTS2018Identifiability_rr}
H.H.M. Weerts, P.M.J. {Van den Hof}, and A.G. Dankers.
\newblock Identifiability of linear dynamic networks.
\newblock {\em Automatica}, 89:247 -- 258, 2018.

\bibitem{pem_joint_direct}
H.H.M. Weerts, P.M.J. {Van den Hof}, and A.G. Dankers.
\newblock Prediction error identification of linear dynamic networks with
  rank-reduced noise.
\newblock {\em Automatica}, 98:256 -- 268, 2018.

\bibitem{YuanGlasso}
M.~Yuan and Y.~Lin.
\newblock Model selection and estimation in regression with grouped variables.
\newblock {\em Journal of the Royal Statistical Society Series B}, 68:49--67,
  02 2006.

\bibitem{yuan2011robust}
Y.~Yuan, G.~Stan, S.~Warnick, and J.~Gon{\c{c}}alves.
\newblock Robust dynamical network structure reconstruction.
\newblock {\em Automatica}, 47(6):1230--1235, 2011.

\bibitem{zhang1993convergence_AIC_BIC}
P.~Zhang.
\newblock On the convergence rate of model selection criteria.
\newblock {\em Communications in Statistics-Theory and Methods},
  22(10):2765--2775, 1993.

\end{thebibliography}

